Detecting Adversarial Patches with Class Conditional Reconstruction Networks

Defending against physical adversarial attacks is a rapidly growing topic in deep learning and computer vision. Prominent forms of physical adversarial attacks, such as overlaid adversarial patches and objects, share similarities with digital attacks, but are easy for humans to notice. This leads us to explore the hypothesis that adversarial detection methods, which have been shown to be ineffective against adaptive digital adversarial examples, can be effective against these physical attacks. We use one such detection method based on autoencoder architectures, and perform adversarial patching experiments on MNIST, SVHN, and CIFAR10 against a CNN architecture and two CapsNet architectures. We also propose two modifications to the EM-Routed CapsNet architecture, Affine Voting and Matrix Capsule Dropout, to improve its classification performance. Our investigation shows that the detector retains some of its effectiveness even against adaptive adversarial patch attacks. In addition, detection performance tends to decrease among all the architectures with the increase of dataset complexity.

==> 4_capnet.tex <==
% \section{Improved CapsNet}
% \label{modifications}

% %\begin{SCfigure}
% \begin{figure}
%     \centering
%     %\vspace{0.7cm}
%     \includegraphics[width=7cm]{figures/CapsulesDropout.pdf}
%     \caption{An abstraction of our modified matrix capsule layer, with MCD (Section \ref{mcd}) and affine voting (Section \ref{affine_voting}).} %Compared to capsules layers in Hinton et al., which uses linear voting without MCD, this converges faster and overfits less.}
%     \label{fig:capsule_layer}
%     %\vspace{-0.8cm}
% \end{figure}

% In this section, we discuss three improvements we made to the architecture of the Capsule Network with EM Routing proposed by Hinton et al.~\cite{hinton2018matrix}, along with empirical evidence on the smallNORB dataset. In particular, we implement i) Matrix-Capsule-Dropout (MCD) layer (Section~\ref{mcd}), ii) Affine voting (Section~\ref{affine_voting}), and iii) Capsule Decoder (Section~\ref{decoder}). To the best of our knowledge, we are the first to attempt dropout and affine voting on matrix capsule layers (Figure \ref{fig:capsule_layer}). The decoder modification is central to our adversarial detection mechanism. %For details regarding the architectures we used for different datasets, please refer to the Appendix in the supplementary materials.
% %
% \subsection{Matrix-Capsule-Dropout}
% \label{mcd}

% \input{tables/mcd}
% {\em Dropout} was proposed by Srivastava et al.~\cite{srivastava2014dropout} in 2014, and since then it has been used in almost all of the state-of-the-art convolutional neural network (CNN) architectures due to its regularizing effects. It approximates ensemble learning in a single dense network by randomly setting neuron activation scalars to zero with probability $p$. The intuition is the same in our implementation of {\em matrix-capsule-dropout} (MCD). If a matrix capsule layer has MCD enabled, then the output capsule activation probabilities of its EM routing procedure during forward propagation will be randomly zero-masked with probability $p$ after the last expectation maximization step.
% %
% This is a computationally inexpensive procedure, as we are only masking the activation probabilities of the capsules without tampering with their matrix representation. In our model, we set $p=0.5$ and apply MCD to randomize the capsule activation probabilities of the second to last and third to last layers in the classification network, so the hidden capsules voting for class capsules in the last layers are deactivated randomly. We are able to {\em reduce over-fitting and improve test accuracy} with this implementation, as shown in Table~\ref{table:dropout_results}. The choices regarding $p$ and affected layers were made without hyperparameter optimization, so better results may be possible. To the best of our knowledge, this is the first work to implement dropout on matrix capsule layers. We also attempted {\em DropRoute}, an adaptation of DropConnect~\cite{wan2013regularization} on the Routing by Agreement mechanism, by randomly assigning routing weights to zero after each expectation maximization step. As we can see from Table~\ref{table:dropout_results}, {\em DropRoute} was not effective.
% %
% %
% \subsection{Affine Voting}
% \label{affine_voting}



% %\setcounter{figure}{1}
% \begin{figure*}
%     \centering
%     %\vspace{-.5cm}
%     \begin{subfigure}{.5\textwidth}
%       \centering
%       \includegraphics[scale=0.175]{figures/affineVSoriginal/t_test.pdf}
%       \caption{Density of differences in test accuracies between 70 and 100 epochs}
%       %; normally distributed (Shapiro-Wilk p=0.840); rejection of hypothesis that differences in epoch test accuracies between 70 and 100 epochs are centered at zero (one-tailed T-test, p=0.010), statistically significant improvement from affine voting.}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}{.5\textwidth}
%       \centering      \includegraphics[scale=0.175]{figures/affineVSoriginal/mean_training_time.pdf}
%       %\label{sp}
%       \caption{Total training time of the two voting mechanisms.}      
%     \end{subfigure}
%     \caption{Affine Voting improves post convergence accuracy and has minimal training time impact.}
%     \label{fig:affineVSoriginal2}
%     %\vspace{-.5cm}
% \end{figure*}



% %\setcounter{figure}{2}
% \begin{figure*}[t!]

% \centering
%     \begin{subfigure}{.5\textwidth}
%       \centering
%       \includegraphics[scale=0.175]{figures/affineVSoriginal/mean_accuracies.pdf}
%       \caption{mean test set accuracies over epochs}
%     \end{subfigure}%
%     \begin{subfigure}{.5\textwidth}
%       \centering
%       \includegraphics[scale=0.175]{figures/affineVSoriginal/median_accuracies.pdf}
%       \caption{median test accuracies over epochs}
%     \end{subfigure}
%     %\vspace{-0.2cm}
% \caption{Affine Voting speeds up convergence. There is a large gap between training sessions using affine voting and linear voting, roughly between epoch 10 to epoch 25. This shows that affine voting capsules are able to converge faster.}
% \label{fig:affineVSoriginal1}
%     %\vspace{-0.5cm}
% \end{figure*}

% Hinton et al. mentions that a lower-level capsule calculates its votes for capsules in the higher levels by ``multiplying its own pose matrix by trainable viewpoint-invariant transformation matrices that could learn to represent part-whole relationships''~\cite{hinton2018matrix}. In other words, votes on higher-layer capsules' pose matrices are linear transformations of lower-layer capsules. Geometrically, the relationships between higher- and lower-layer capsule poses estimated by those linear votes are compositions of rotations, reflections, and scaling. On the other hand, our architecture calculates the votes through {\em affine transformations}, which multiplies a pose matrix with a trainable transformation matrix, followed by addition of a trainable bias matrix. While this is partly inspired by the use of bias terms in CNNs, geometrically affine transformations can model compositions of rotations, reflections, and scaling, followed by translations. Thus, they are strictly more expressive than that of the default linear transformations proposed in the {\em EM Routing} paper, and can model more general relationships between higher and lower level capsules. This comes at the cost of doubling the amount of trainable parameters in capsule layers with all else unchanged. 
% %
% To evalaute the effect of affine transformations, we compared the training and testing performances of {\em linear voting} and {\em affine voting} on the smallNORB dataset, with ten training sessions for each voting mechanism. We find that affine voting significantly increases post-convergence accuracy. In Figure~\ref{fig:affineVSoriginal2}a, we illustrate the empirical density of differences in test accuracies between affine voting and linear voting in the range from 70 and 100 epochs, where the training has converged. The density is normally distributed (Shapiro-Wilk p=0.840), and we find a statistically significant improvement for affine voting, as indicated by a rejection of the hypothesis that the differences are centered at zero (one-tailed T-test, p=0.010). Furthermore, affine voting only increases the time per epoch by about 2\% (Figure~\ref{fig:affineVSoriginal2}b),
% %, we conclude that affine voting does not noticeably increase iteration time per training epoch (Figure~\ref{fig:affineVSoriginal2}a), while increasing post convergence accuracy (Figure~\ref{fig:affineVSoriginal2}b), and significantly 
% while speeding up convergence overall by reducing the number of training epochs needed to get good accuracies (Figure~\ref{fig:affineVSoriginal1}). Note that our training times reached over 60 hours for 100 epochs, so the trade-off of lower accuracy for a faster training time may be worth it in some applications.

% %\textcolor{blue}{\textbf{Saidur - I don't see any difference between the affine and linear voting in Figure 3. Can you explain more to justify your statement? Perry - I have added more explanation.}}


% %
% \if 0
% \begin{SCfigure}
% \includegraphics[scale=0.225]{figures/badrecon/background.jpg}
% \caption{Background Capsules encode more than background (Left: CIFAR10 Input image, Middle: Reconstructed image, Right: Reconstructed image with background Capsule activation zeroed). We can see that when background capsules are deactivated on the right, the object in the center also loses fidelity. This would not be the case if our background capsules only encode information for background as intended.}
% \label{fig:background_recon}
% \vspace{-0.4cm}
% \end{SCfigure}
% \fi
% %We also explored the use of unsupervised background classes for reconstruction to potentially improve its performance in classification datasets that are not pre-segmented, by adding in additional class capsules activations that are not part of the classification loss. We feed the capsule matrices of these activations into the reconstruction network. The results of this approach are inconclusive, as the background classes learned to encode more than just background information. The architecture also seems to be more prone to adversarial patching when there are background capsules, resulting in a higher rate of classification fooling and detection evasion, although this might result from randomness. Hence for our experiments in Section~\ref{adv_experiments}, we implemented the decoder without background capsules even in non-segmented datasets (CIFAR10 and SVHN). Some examples of reconstruction with background class capsules are shown in Figure~\ref{fig:background_recon}.

% %\textcolor{blue}{\textbf{Saidur - Can you explain more what we are seeing from the Fig 4. Perry - I have added more explanation in the caption}}


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> figures/background_figs.tex <==
\begin{figure}[t]
%\centering
    \begin{subfigure}{1\textwidth}
      \centering
      \includegraphics[scale=0.20]{figures/badrecon/fig2.png}
      %\includegraphics[width=1\linewidth, height=75px]{figures/badrecon/Figure_2.png}
    \end{subfigure}%
    
    \begin{subfigure}{1\textwidth}
      \centering
      \includegraphics[scale=0.20]{figures/badrecon/fig6.png}
      %\includegraphics[width=1\linewidth, height=75px]{figures/badrecon/Figure_6.png}
    \end{subfigure}
    
    \begin{subfigure}{1\textwidth}
      \centering
      \includegraphics[scale=0.120]{figures/badrecon/fig7.png}
      %\includegraphics[width=1\linewidth, height=75px]{figures/badrecon/Figure_7.png}
    \end{subfigure}
    \caption{Background Capsules encode more than background (Left: CIFAR10 Input image, Middle: Reconstructed image, Right: Reconstructed image with background Capsule activation zeroed). We can see that when background capsules are deactivated on the right, the object in the center also loses fidelity. This would not be the case if our background capsules only encode information for background as intended.}
    \label{fig:background_recon}
    \vspace{-0.5cm}
\end{figure}
